Autonomous Passage Planning for a Polar Vessel

We introduce a method for long-distance maritime route planning in polar regions, taking into account complex changing environmental conditions. The method allows the construction of optimised routes, describing the three main stages of the process: discrete modelling of the environmental conditions using a non-uniform mesh, the construction of mesh-optimal paths, and path smoothing. In order to account for different vehicle properties we construct a series of data driven functions that can be applied to the environmental mesh to determine the speed limitations and fuel requirements for a given vessel and mesh cell, representing these quantities graphically and geospatially. In describing our results, we demonstrate an example use case for route planning for the polar research ship the RRS Sir David Attenborough (SDA), accounting for ice-performance characteristics and validating the spatial-temporal route construction in the region of the Weddell Sea, Antarctica. We demonstrate the versatility of this route construction method by demonstrating that routes change depending on the seasonal sea ice variability, differences in the route-planning objective functions used, and the presence of other environmental conditions such as currents. To demonstrate the generality of our approach, we present examples in the Arctic Ocean and the Baltic Sea. The techniques outlined in this manuscript are generic and can therefore be applied to vessels with different characteristics. Our approach can have considerable utility beyond just a single vessel planning procedure, and we outline how this workflow is applicable to a wider community, e.g. commercial and passenger shipping.

==> Sections/smoothingalgorithm.tex <==
\begin{algorithm}[H]
\bf{Algorithm: smoothThePaths(R,T,P)}\\
\KwData{A mesh of the region R for time period T, A list of Dijkstra paths, P}
\KwResult{C: A list of smoothed paths, one for each Dijkstra path in P}
\Begin{
\For{p \Kwin P}
{
\While(!converged){
List adjs = Extract the adjacent cell pairs of $\mathcal{p}$\
LatLong startwp = the start waypoint of p\
LatLong endwp = the end waypoint of p\ 
LatLong firstpoint = startwp\
LatLong midpoint = null\
LatLong lastpoint = null\ 
\For{ap \Kwin adjs}

\If(ap.rbox = ap.lbox){
remove reversed edges\ 
}

midpoint = ap.getYLatLon\
lastpoint = endwp if this is the last ap otherwise apnext.getYLatLon  \ 

\If(abs(firstpoint-midpoint) < MERGESEP){
firstpoint = midpoint\ 
midpoint = lastpoint\ 
lastpoint = endwp if this is the last ap otherwise apnext.getYLatLon  \ 
}

\If(abs(midpoint-lastpoint) < MERGESEP){
retrieve the next adjacent cell pair, apnext\ 
midpoint = ap.getYLatLon\ \ 
lastpoint = endwp if this is the last ap otherwise apnext.getYLatLon  \ 

}

int di = ap.direction\ 

\If(di is a diagonal)

double latcross\ 
double longcross\ 
double latdiff\ 
double longdiff\ 


\If(latdiff > longdiff){
remove ap from adjs\ 
\If(latcross > longcross){
    
    add bottom left cell and two new aps in directions -2 and -4\ 
}
\Else{
    add top right cell and two new aps in directions 2 and 4\ 
}
}
\Else{
\If(latcross > longcross){
    
    add bottom right cell and two new aps in directions -2 and 4\ 
}
\Else{
    add top left cell and two new aps in directions 2 and -4\ 
}
}
\If(dif!=0){
\If(there are neighbours in the dif direction){
remove ap\ 
add a new ap in direction dif\ 
}
\Else{
clip to the lbox corner\ 
}
}
\Else{
\If(dit!=0){
\If(there are neighbours in the dit direction){
remove ap\ 
add a new ap in direction dit\ 
}
\Else{
clip to the rbox corner\ 
}
}
}
\Else{
create a horseshoe\ 
}
}

add new path p to C\ 
   

\Return{$\mathcal{C}$}\;

}
}

\caption{Subdivide Cell, $C$ into partitions according to homogeneity condition, $H$, applied to content data $D$.}\label{alg1}
\end{algorithm}
